SCAR: Scheduling Multi-Model AI Workloads on Heterogeneous Multi-Chiplet Module Accelerators

Emerging multi-model workloads with heavy models like recent large language models significantly increased the compute and memory demands on hardware. To address such increasing demands, designing a scalable hardware architecture became a key problem. Among recent solutions, the 2.5D silicon interposer multi-chip module (MCM)-based AI accelerator has been actively explored as a promising scalable solution due to their significant benefits in the low engineering cost and composability. However, previous MCM accelerators are based on homogeneous architectures with fixed dataflow, which encounter major challenges from highly heterogeneous multi-model workloads due to their limited workload adaptivity. Therefore, in this work, we explore the opportunity in the heterogeneous dataflow MCM AI accelerators. We identify the scheduling of multi-model workload on heterogeneous dataflow MCM AI accelerator is an important and challenging problem due to its significance and scale, which reaches O(10^56) even for a two-model workload on 6x6 chiplets. We develop a set of heuristics to navigate the huge scheduling space and codify them into a scheduler, SCAR, with advanced techniques such as inter-chiplet pipelining. Our evaluation on ten multi-model workload scenarios for datacenter multitenancy and AR/VR use-cases has shown the efficacy of our approach, achieving on average 27.6% and 29.6% less energy-delay product (EDP) for the respective applications settings compared to homogeneous baselines.

==> Algorithms/layer_assignment_simp.tex <==
% Section 4.2
\begin{algorithm}[H]
\caption{Layer Assignment}\label{alg:layer_assign}
\begin{algorithmic}[1]
    \Require{$W$ (Workloads), $P_{\text{Strat}}$ (partition strategy), $C$ (chiplet classes), $|\mathbb{C}|$ (\# of chiplets), $n_{c_{i}}$ (\# of class $i$ chiplets)}
    \Ensure{$L2W$ (Layer(s) to execution windows assignments)}
    \Function{LayerAssignment}{$W$, $P_{\text{Strat}}$, $C$, $|\mathbb{C}|$, $n_{c_{i}}$}
        \For{$\mathcal{NN} \in W$}
            \State $exec\_win, wind\_idx, used\_cycles = (), 0, 0$
            \For{$l \in \mathcal{NN}$}
                \LineComment{\% expected layer execution latency on chiplet class $i$}
                \State $\mathbb{E}(Lat(l)) = \sum_{i=1}^C \frac{n_{c_{i}}}{|\mathbb{C}|}\times Lat(l\rightarrow i)$
                \While{True}
                    \State $last = wind\_idx == |P_{\text{Strat}}|$
                    \LineComment{\% entire expected $\mathcal{NN}$ latency fits in $wind\_idx$}
                    \State $fits = \mathbb{E}(Lat(\forall l \in \mathcal{NN})) < P_{\text{Strat}}[wind\_idx]$
                    \If{$last$ or $fits$} 
                    \State $exec\_win$ += $l$
                    \State $used\_cycles$ += $\mathbb{E}(Lat(l))$
                    \State \textbf{Break}
                    \Else      
                    % \LineComment{\% remaining execution time}
                    \State $Slack$ = $P_{\text{Strat}}[wind\_idx] - used\_cycles$ 
                        \If{$\mathbb{E}(Lat(l)) <= Slack$}
                            \State $exec\_win$ += $l$
                            \State $used\_cycles$ += $\mathbb{E}(Lat(l))$
                            \State \textbf{Break}
                        \Else 
                        % \LineComment{\% continue assignment at next execution window}
                            \State $L2W[win\_idx][\mathcal{NN}] = exec\_win$ 
                            % \LineComment{\% current execution window layer assignments for $\mathcal{NN}$}
                            \State $used\_cycles = P_{\text{Strat}}[wind\_idx]$
                            \State $exec\_win = ()$
                            \State $wind\_idx$ += 1
                        \EndIf
                    \EndIf
                \EndWhile
            \State $L2W[win\_idx][\mathcal{NN}] = exec\_win$ 
            % \LineComment{\% current execution window layer assignments for $\mathcal{NN}$}
            \EndFor
        \EndFor
        \State \Return{L2W}
    \EndFunction
\end{algorithmic}
\end{algorithm}

==> Algorithms/provisioner.tex <==
\begin{algorithm}[H]
\caption{Resource Provisioning}\label{alg:provis}
\begin{algorithmic}[1]
    \footnotesize
    \Require{$|\mathcal{C}|$ (\# of chiplets), $n_{df_{i}}$ (\# dflow $i$ chiplets), $L2W$ (layer assigns), $\mathbb{P}$ (overall expected compute efforts)}
    \Ensure{$Alloc$ (node allocations per window per model)}
    \Function{Provisioner}{$|\mathcal{C}|$, $n_{df_{i}}$, $L2W$, $\mathbb{P}$}
        \State $Alloc = ()$
        \For{$exec\_win \in L2W$}
            \State $\mathbb{P}_{win} = \mathbb{P}[exec\_win]$
                \For{$\mathbb{E}(\mathcal{P}_j) \in \mathbb{P}$}
                    \LineComment{\% Preliminary allocation}
                    \State $Alloc$ += ($round(\frac{\mathbb{E}(\mathcal{P}_{j})}{\sum^{|\mathbb{P}|}_{k}(\mathbb{E}(\mathcal{P}_{k})} \times |\mathcal{C}|), )$
                \EndFor
            \EndFor
            \LineComment{\% Ensure at least one resource per workload}
            \While{$\exists$ $Alloc_{j} \in Alloc$ s.t. $Alloc_{j}=0$}
                \State $Alloc_{k} = max(Alloc)$ s.t. $Alloc_{k} \neq Alloc_{j}$
                \State $Alloc_{j} = ReAlloc(Alloc_{k})$
            \EndWhile
        \State \Return{$Alloc$}
    \EndFunction
\end{algorithmic}
\end{algorithm}

==> Algorithms/top_level.tex <==
% Section 4.2
\begin{algorithm}[H]
\caption{Top Level}\label{alg:top}
\begin{algorithmic}[1]
    \Statex \red{"in progress; will replace some text"}
    \Require{$W$ (Workloads), $P_{\text{Strat}}$ (partition strategy), $C$ (chiplet classes), $|\mathbb{C}|$ (\# of chiplets), $n_{c_{i}}$ (\# of class $i$ chiplets)}
    \Ensure{$L2W$ (Layer(s) to execution windows assignments), $N$ (node allocations per $exec\_win$ per model)}
    \Function{Top Level}{$W$, $P_{\text{Strat}}$, $C$, $|\mathbb{C}|$, $n_{c_{i}}$}
        \LineComment{\% Window Assignments}
        \For{$\mathcal{NN} \in W$}
            \State $exec\_win, win\_idx, used\_cycles = (), 0, 0$
            \For{$l \in \mathcal{NN}$}
                \LineComment{\% expected layer execution latency on chiplet class $i$}
                \State $\mathbb{E}(Lat(l)) = \sum_{i=1}^C \frac{n_{c_{i}}}{|\mathbb{C}|}\times Lat(l\rightarrow i)$
                \While{True}
                    \State $last = wind\_idx == |P_{\text{Strat}}|$
                    \LineComment{\% entire expected $\mathcal{NN}$ latency fits in $win\_idx$}
                    \State $fits = \mathbb{E}(Lat(\forall l \in \mathcal{NN})) < P_{\text{Strat}}[win\_idx]$
                    \If{$last$ or $fits$} 
                    \State $exec\_win$ += $l$
                    \State $used\_cycles$ += $\mathbb{E}(Lat(l))$
                    \State \textbf{Break}
                    \Else      
                    % \LineComment{\% remaining execution time}
                    \State $Slack$ = $P_{\text{Strat}}[win\_idx] - used\_cycles$ 
                        \If{$\mathbb{E}(Lat(l)) <= Slack$}
                            \State $exec\_win$ += $l$
                            \State $used\_cycles$ += $\mathbb{E}(Lat(l))$
                            \State \textbf{Break}
                        \Else 
                        % \LineComment{\% continue assignment at next execution window}
                            \State $L2W[win\_idx][\mathcal{NN}] = exec\_win$ 
                            % \LineComment{\% current execution window layer assignments for $\mathcal{NN}$}
                            \State $used\_cycles = P_{\text{Strat}}[win\_idx]$
                            \State $exec\_win = ()$
                            \State $win\_idx$ += 1
                        \EndIf
                    \EndIf
                \EndWhile
            \State $L2W[win\_idx][\mathcal{NN}] = exec\_win$ 
            % \LineComment{\% current execution window layer assignments for $\mathcal{NN}$}
            \EndFor
        \EndFor
        \LineComment{\% Resource Provisioning}
        \For{$win\_idx \in enum(P_{\text{Strat}})$}
            \For{$j \in W$}
                \LineComment{\% Expected compute effort $\mathcal{P}$ on chiplet class $i$}
                \State $\mathcal{P}_{j} = L2W[win\_idx][j]$
                \State $\mathbb{E}(\mathcal{P}_{j}) = \sum_{i=1}^C \frac{n_{c_{i}}}{|\mathbb{C}|}\times \mathcal{P}_{j} \rightarrow i)$
                \LineComment{\% Preliminary allocation}
                \State $Alloc_{j}$ = $round(\frac{\mathbb{E}(\mathcal{P}_{j}))}{\sum^{W}_{k}(\mathbb{E}(\mathcal{P}_{k}))} \times |\mathbb{C}|)$
            \EndFor
            \LineComment{\% Resource balancing}
            \While{$\exists$ $Alloc_{j} \in Alloc$ s.t. $Alloc_{j}=0$}
                \LineComment{Find largest resource allocations candidate}
                \State $Alloc_{i} = max(Alloc)$ s.t. $Alloc_{i} \neq Alloc_{j}$
                \LineComment{ensures at least one resource per model per window}
                \State $Alloc_{j} = ReAlloc(Alloc_{i})$
            \EndWhile
            \EndFor
        \State \Return{L2W, $Alloc$}
    \EndFunction
\end{algorithmic}
\end{algorithm}

==> Include/packages.tex <==
% \usepackage{cite}

\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts, amsthm}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage[hyphens]{url}
\usepackage{fancyhdr}
\usepackage[bookmarks=true,breaklinks=true,letterpaper=true,colorlinks,citecolor=blue,linkcolor=blue,urlcolor=blue]{hyperref}

\usepackage{multirow}

\usepackage{algorithm}
% \usepackage{algpseudocode}
%% removes end conditions
\usepackage[noend]{algpseudocode}

\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}


\RequirePackage[nameinlink]{cleveref} % 'nameinlink' to mimic \autoref's behavior
%% Use low-level controls to hard-code the required appearance.
\crefname{chapter}{Chapter}{Chapters}
\crefname{section}{Section}{Sections}
\crefname{subsection}{Section}{Sections}
\crefname{equation}{Equation}{Equations}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithms}
% etc
\let\autoref\cref % set \autoref as an alias for \cref

==> Sections/03_Problem_Formulation.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}

We formulate the scheduling problem of multi-model workloads on MCM with heterogeneous dataflow chiplets. 

\subsection{Base Formulation}

Define ${M}$ = \{$m_1, m_2, ..., m_n$\} as a multi-model inference workload, where each model $m_j$ is defined by a topologically sorted set of layers based on the layer dependency given by: $m_j=\{l^{j}_1, l^{j}_2, \cdots, l^{j}_{L_j}\}$, with $L_j$ being the total number of layers of $m_j$. Each $l^{j}_r$ represents the $r^{th}$ topologically sorted layer defined through its parameters as:
\begin{equation}
\abovedisplayskip=0pt
    l^{j}_r = (batch\_size, C_{in}, C_{out}, ip\_size, k\_size)
\belowdisplayskip=5pt
\end{equation}
where these parameters represent the respective batch sizes, the number of input channels, the number of output channels, input resolution (h, w), and the kernel size.

We formulate the heterogeneous dataflow MCM package as follows: 
\begin{equation} 
\abovedisplayskip=0pt
MCM = (\mathcal{C}, NoP, hw\_params)
\belowdisplayskip=5pt
\end{equation} 
where $\mathcal{C}$ = \{$c_1, c_2, \cdots, c_n\}$ is a set of chiplets integrated onto the MCM package ($MCM$),
$NoP$ characterizes the network-on-package and the underlying connection topology (e.g., mesh) linking the on-package chiplets together and with the memory nodes via silicon interposer. $hw\_params$ pertain to the hardware parameters characterizing the MCM package from the individual components (e.g., chiplet die sizes.). For each accelerator chiplet $c \in \mathcal{C}$, it can be defined by its own parameters:
\begin{equation}
\abovedisplayskip=0pt
c = (\#pes, L1\_mem, L2\_mem, NoC, df)
\belowdisplayskip=5pt
\end{equation}
where $\#pes$ represents the number of processing engines ($pes$) within an accelerator chiplet, with $L1\_mem$ being its local memory size; $L2\_mem$ is the global shared buffer size across all pes. $NoC$ is the network-on-chip characterizing its associated topology and parameters (e.g., bandwidth). $df$ represents the dataflow supported on the chiplet $c$. We denote $DF = \{df_1, df_2, \cdots, df_n\}$ as the set of $n$ unique heterogeneous dataflows associated with every $c \in \mathcal{C}$.

\subsection{Heterogeneous MCM Scheduling Problem}

Given the base formulations, the goal is to optimize the scheduling strategy for the set of multi-model workloads on the shared MCM such that performance efficiency with regards to a target metric (e.g., EDP) is maximized. Given the multi-faceted spatio-temporal considerations of the multi-model MCM scheduling problem, we define it as a bi-level optimization problem: (1) \textbf{At the top level, the goal is to optimize for $\rho$; a time partitioning strategy} specifying the times at which a reconfiguration of the MCM chiplets is to be enacted (i.e., characterizing the start and end times of independent shared execution windows). (2) \textbf{At the inner level instantiated for each window, the goal is to optimize $\alpha$; the scheduling strategy} concerning actual resource allocation and mapping of chiplets to multi-model workloads. Formally, the optimization problem is given as:%\footnote{we slightly abuse using the total number index notation `$n$' across formulas}:

\begin{align}
\abovedisplayskip=0pt
    \rho^{*} = \max_{\rho} &\mathcal{P}(\rho \vert \{\alpha^{*}_0, \cdots, \alpha^{*}_{n_{splits}}\}, \{M_0,\cdots, M_{n_{splits}}\}) \label{eqn:out}\\
    s.t., \alpha_i^{*} =& \max_{\alpha} \mathcal{P}_{inr} (\alpha | M_i, MCM) \label{eqn:inr} \\
    where
    \;\; \rho =& \{t_{s_1}, t_{s_2}, \cdots, t_{s_{n_{splits}}}\}, \label{eqn:partn} \\
    M_i =& \{m_1^i, m_2^i, \cdots, m_n^i\} \;s.t., m_j^{i} \subset m_j \label{eqn:par-model}\\
    \alpha_i =& (l_r^{ij} \rightarrow c_k \;|\; c_k \in \mathcal{C} \;\forall l_r \in m_j^{i}) \label{eqn:layer-assign}\\
    s.t.,& c_k \neq c_u \forall l_r^{ij} \rightarrow c_k \land l_{r'}^{ij'} \rightarrow c_u, j\neq j' \label{eqn:assign_cnstr}
    % map(\cdot) =& f(l_^{j} \in m^i \rightarrow c_j \in \mathbb{C})
    % \{P(s_i^{*} \vert \mathbb{M}_{i}, MCM\}] \label{eqn:outer} \\ 
    % s.t. \; s^{*} = \max_{s\in\mathbb{S}}P(s\vert \alpha, \mathbb{CU}) \label{eqn:inner}
\end{align}


% naturally this characterizes a shared window basis for all the models, losing some granularity at the expense of structured problem definition

where $p^{*}$ in the outer optimization formula (\ref{eqn:out}) represents the optimal partitioning strategy maximizing the target performance objective function $\mathcal{P}$, conditioned on optimal per-window schedules $\{\alpha_i^{*}\}$, and sub-models assignments to windows $\{M_i\}$. Starting with the latter, each $M_i \in \{M_i\}$ characterizes a subset of layers from each $m_j \in M$ that are assigned to the $i^{th}$ execution window as shown in equation (\ref{eqn:par-model}). These execution windows are the outcome of each partitioning strategy $p$. where as seen in equation (\ref{eqn:partn}), each $p$ is defined by a set of splitting points, $\{t_{s_{j}}\}$, where each $t_{s_{j}}$ indicates a discrete boundary point separating two adjacent execution time windows with $s_j$ indicating the $j^{th}$ splitting point.

As for the optimal schedule $\alpha_i^{*}$ per window $i$ defined in equation (\ref{eqn:inr}), it represents the schedule $\alpha$ that maximizes the per-window performance evaluation function, given by $\mathcal{P}_{inr}$, conditioned on $M_i$ and the underlying MCM characterization. In more detail as shown in equation (\ref{eqn:layer-assign}), $\alpha$ is concerned with the assignment of each layer $l_r^{ij}$ from sub-model $m_j^{i}$ to a chiplet $c_k \in \mathcal{C}$, where within a single window, no two layers from different sub-models models are allowed to share the same chiplet to maximize per-window locality, leaving temporal allocations of chiplet resources across models to be handled through the specification of time windows from $\rho$.

\betterparagraph{Summary} The outer optimization formula handles the MCM reconfiguration strategy with regards to revisiting the resource allocation strategy across the multi-model workloads depending on their computational footprints in each time window. The inner optimization formula handles the mechanics of spatially mapping the sub-model workloads to the underlying heterogeneous chiplets, considering MCM features of dataflow affinities and inter-layer pipelining to maximize the overall per-window performance efficiency. In the following Section, we discuss our proposed scheduling framework implemented to navigate the complex scheduling search space characterized by this system model.



% naturally, the reason for such stalling latency and not wait for the entire time window is to benefit from heterogeneity,



% where the inner optimization level is concerned with the \textit{spatial} resource distribution of chiplets across the various multi-model workloads, as well as the corresponding mapping problem. The outer level is more concerned with a \textit{temporal} aspect of the scheduling in which we determine points in the discrete time space at which a reconfiguraiton of the MCM resources can be enacted. 






% \OD{Evaluation and optimization from the top level engine to be always based on LATENCY. Any other optimization level can use LAT, ERGY, and EDP}

% Given a shared multi-chiplet module (MCM) comprising $K$ chiplets arranged in a 2D tiled chiplet-array with access to a DRAM memory resources, and given a set of $N$ multi-model neural network workloads, $\mathcal{NN}$, requesting computational service by the MCM module, the scheduling problem of mutli-model workloads onto a MCM to optimize a target performance metric (e.g., inference latency, energy, or EDP) can be viewed as a two-level optimization problem: (1) The first is to identify points along the execution time axis of the involved multi-models at which the allocation of chiplet resources to models can be revisited, which we refer to as \textit{MCM reconfiguration times}. Through this characterization of MCM reconfiguration times, we obtain separate execution windows within which the inner level of optimization can be applied. (2) The inner optimization level, conditioned on a given execution window characterization, is concerned with identifying the optimal allocation strategies of different chiplets to different workload layers so as to realize schedules improving on a certain performance metric. 

% This model leaves several considerations to be engaged, as in within each window, what layers from each workload should be assigned to which window? what is the assignment criteria? How to take layer affinities to dataflows into consideration? How can we rank and compare configurations at such a high-level considering the uncertainty of the final chiplets to layers assignment? How can we embed parallel execution features such as inter-layer and -chiplet pipelining within our decision-making and evaluation? In this context, designing an optimization framework under such uncertainties would require achieving an intricate balance between design space exploration, heuristics application, and evaluation confidence. 


% \OD{from here starts an old draft}

% From here, an effective scheduling approach ilicits a requirement for a unified system model that captures the various runtime execution scenarios that can be encountered in the deployment environment. Specifically, a unified model considers \textit{\textbf{(1) the multi-model neural network workloads;}} specifically their execution characteristics given how each model constitutes a distinctive computational DAG structure with different resource requirements, kernel affinities, and varying degrees of computational complexities, leading both the \textit{number} and \textit{class} of workloads to influence the scheduling effectiveness. For instance, two models of different classes (e.g., a CNN and an LLM) can be competing for the same resources to serve their respective applications. In such cases, it is not necessarily ideal to distribute resources equally between the two models, rather it can be beneficial to allocate more resources to the LLM considering the magnitude and complexity of its underlying operations. A different use case can be encountered when the same application instantiates different models, possibly of different classes, in a sequential manner, as is the case with AR/VR applications (e.g., hand detection then hand tracking), or such as the generative AI features embedded within image application, such as stable diffusion relying on a UNet backbone for segmentation task conditioned on a transformer output. Another Scenario when $N$ > $k\times k$, requires support for a temporal scheme of resources' allocation to the competing workloads, where over the course of a time segment in which $N$ remains the same and greater in number than the available resources, flushing and refetching may be performed frequently across the accelerator tiles to ensure a fair service for the competing workloads. \textbf{\textit{(2) The allocation of chiplet resources and reconfigurability;}} where the goal is to maximize utilization of resources, minimize data movements, and support applications to meet their processing deadlines. As mentioned above, the allocation of resources should be customized to suit the $N$ workloads at the scheduling queue in order to allow them to leverage data locality, parallelism, and low-cost access to memory without affecting the other workloads. However, as the computational footprints of the different models begin to change (e.g., feature map spatial dimensions are reduced within a CNN), and some models $N' \in N$ conclude processing, a redistribution of chiplets can be instantiated to allocate more resources to the remaining workloads. \textbf{\textit{(3) Data Movement and Computation;}} For each chiplet resource, the choices of \textit{intra-layer parallelism} parameters (e.g., dataflow and tiling sizes) must factor in the overall cost characterization for processing the designated layers, as well the \textit{inter-layer parallelism } in which the output feature maps are either retained on the same chiplet for the following layer to be executed on the same chiplet (layer sequential parallelism), or partial outputs are immediately forwarded to a nearby chiplet hosting the subsequent layers using the NoP configuration for continued processing in a pipelined fashipn (layer pipelining parallelism). Otherwise, data would need to be written back and refetched to the main memory for reuse by the following layers. Based on this high-level overview, the following subsection breaks down the constituent building blocks for achieving the desired properties out of the scheduling problem while abiding by the system constraints. 

% \subsection{Scheduler System Model}
% \red{Initial terminology to be refined}
% To effectively map the multi-model multi-modal neural workloads, $\mathcal{NN} = \{nn_1, nn_2, \cdots, nn_N\}$, onto the MCM chiplets, $CU = \{cu_1, cu_2, \cdots, c_K\}$, a scheduler is to be designed with support for the functionalities specified through the blocks in Figure \ref{fig:building_blocks}. Here, the scheduling granularity is performed on the chiplet level, that is, the combination of processing engines, L2 buffers belonging to each chiplet are treated as a single monolithic resource that can service one or more layers. Given a schedule optimization time horizon of $T_H$ ending with the last executable layer of any model $\forall nn \in \mathcal{NN}$. The functionalities correspond to the aforementioned blocks described in the following.

% \textbf{Workloads Parser.} Firstly, workloads characterizing the set of $N$ models in a corresponding scheduling horizon, $T_h$, are parsed and added to the set $CG$=$\{cg_1, cg_2, \cdots, cg_N\}$, where each $cg_i$ indicates the computational graph for the $i^{th}$ model workload capturing the operational and data dependencies  across the constituent layers in each model needed to construct a computing schedule. Given a default configuration of chiplet hardware parameters and dataflow, an initial estimation of each layer computational is also determined. 

% \textbf{Execution Times Partitioner (ETP).} Given how each $cg_i$ comprises a unique composition of computational kernels, graph topologies, intermediate features sizes, memory access patterns, and dataflow affinities, the ETP is tasked with identifying the subset of time points $T_{par} \subset T_H$ at which the allocation of chiplet resources, $CU$, to models, $\mathcal{NN}$, can be reconfigured for better projected performance. I.e., the ETP's responsibility is to act as a dynamic resource allocater of the chiplet resources at certain pre-determined times. As such, the ETP first constructs a space of potential regrouping time points based on a prespecified criteria. For instance, the spacing between candidate regrouping time points can be set based on the largest execution time for any layer $l_i \in nn_i \forall nn_i \in \mathcal{NN}$. A finer or coarser granularity can always be defined, which is to be reflected on the search complexity. From the ETP, we obtain $T_{par}$=$\{T_1, T_2, \cdots, T_m\}$ with each $t_i$ indicates the $i^{th}$ regrouping point.

% \textbf{Spatial Grouper (SG).} For every $t_i \in T_{par}$, the LG explores for each model, $nn_j$, which subset of layers, $L_m$, should be grouped together for assignment onto the same subset of chiplets. This facilitates the exploitation of data locality across successive layers, and enables the support for both pipelining and shared memory parallelism in the inner scheduler, all while maintaining separate processing domains for each workloads across the temporal and spatial dimensions. The minimum number of layer groups at any time is equivalent to $|\mathcal{NN}|$ assuming the workloads in $\mathcal{NN}$ are independent. On the other hand, the maximum number of groups is obtained when each layer is assigned a separate group. The return from LG is a set of layer groups $G =\{g_1, g_2, \cdots, g_{n'} \}$ where $n'$ is the index of the final group upper bounded by the number of layers assigned for processing in the $i^{th}$ regrouping window.

% \textbf{Temporal Grouper (TG).} Given the possibility of attaining a scenario in which $|\mathcal{NN}|$ > $|CU|$, temporal multiplexing is adopted to ensure a fair sharing scheme of the chiplet resources amongst all models, adding another dimension to the resource allocation optimization strategies. For instance, an equal workload/chiplet distribution across the spatial and temporal dimensions may not necessarily be the optimal configuration given the heterogeneity of model operations and execution characteristics.  

% \textbf{Chiplet Logical Grouper.} On the level of hardware, the various possibilities of logical chiplet groupings are characterized as the design space in the chiplet logical grouper for determining the best schedule of workloads onto chiplets. The grouper covers all possibilities of 2D Meshes, adjacent horizontal or vertical grouping, as well as standalone options. Formally, the logical chiplet clusters can be given by $C = \{c_1, c_2, \cdots, c_{m'}$, where $m'$ indicates the number of chiplet groups for this corresponding window, upper bounded by the total number of chiplets $|CU|$. The logical groups are constructed according to the chiplets' physical geometric proximity. 

% \textbf{Outer Inter-Group Scheduler (OS).} Given $G$ and $C$, the outer scheduler performs the first mapping of every $g_i \in G$ onto one of the chiplet groups in $C$. The mapping would take into consideration the layer groups' demands, data locality, and previous assignments. Each layer group is processed separately on its chiplet group independent of other workloads.

% \textbf{Inner Intra-Group Scheduler (IS)} Given $G$ and $C$, the final block is tasked with assigning every $l_i \in g_j$ to a chiplet $cu_m \in c_k$. Through IS, pipelining and sequential parallelism options can be explored for the layer groups within. This finer scheduling granularity considers how data moves between chiplets belonging to the same cluster, and where the final results are accumulated before being pushed back onto the main memory. The output is a vector of mapping vectors in which $l_i \rightarrow cu_j \forall (l_i, cu_j) \in (g_i, c_j)$.

==> Sections/evaluation_b4_overhaul.tex <==
\section{Evaluation}
\label{sec:eval}

\subsection{Experimental Settings} \label{subsec:settings}

\input{Tables/scenarios}

\begin{figure}[!tbp]
\begin{center}
{\includegraphics[,width = 0.48\textwidth]{Figures/patterns2.pdf}}
\end{center}
\vspace{-2.6ex}
\caption{\blue{Evaluated MCM chiplet organizations in this work.}}
\label{fig:pattrn}
\vspace{-1ex}
\end{figure}

\betterparagraph{Multi-Model Workloads}
Our evaluations are performed on multi-model workload scenarios based on models from (1) MLPerf inference benchmark \cite{reddi2020mlperf, mlcommons}, which are curated for datacenter multi-tenancy setting following data
center usage trends in \cite{hazelwood2018applied, park2018deep, jouppi2017datacenter}. (2) XRBench \cite{kwon2023xrbench} for multi-model AR/VR workloads. The full list of scenarios is provided in Table \ref{tab:scenarios} covering a wide range of use-cases with varying degrees of diversity and complexity. 

%We implement our MLPerf following datacenter usage trends in \cite{hazelwood2018applied, park2018deep, jouppi2017datacenter}. 

% \red{In the AR/VR scenarios, the nature of search resources means that we trade-off search space granularity for complexity. That is, chunks of layers will be assigned to one chiplet or the other based on the dominant layer in a sequence (e.g., DW conv may be dominant in the latter layers, tilting its sequence towards os, but at low resolution, ws might be the one preferred for all.}

% we implement 5 inference scenarios reflecting an incremental rise in both computational complexity and model diversity. For each scenario, we include at least two LLM workloads following the current AI trend. Unless otherwise stated, Scneario 4 is the default.

\betterparagraph{MCM System} Our default MCM systems follows the Simba architecture \cite{shao2019simba}. Simba comprises a total of 36 chiplets connected through a Mesh topology and arranged as four $3\times3$ groups of chiplets. We implement (1) $3\times3$, and (2) $6\times6$ MCM templates for our experiments. we adopt XY routing for on-pacakge data movement, and integrate further memory interfaces on the sides of the outer chiplets, providing direct links to the offchip DRAM via double-sided memory channels as in \cite{gao2019tangram}. We consider 4096 PEs/chiplet and 256 PEs/chiplet for the datacenter and AR/VR settings, respectively. We set the L2 shared memory size in each chiplet to 10 MB, inspired by the on-chip memory size in a recent mobile accelerator~\cite{qualcomm_hexagon_680}.

\betterparagraph{Baselines and Heterogeneity Patterns}
We choose Shidiannao \cite{du2015shidiannao} and NVDLA \cite{nvdla} dataflow styles for our accelerator chiplets and adopt two baselines:
\begin{itemize}
    \item \textit{Standalone}. each model is assigned a single accelerator chiplet - all chiplets adopt the same dataflow.
    \item \textit{Simba-like Pipelining}. In each time window, model workloads can be assigned to more than one chiplet. All chiplets adopt the same dataflow.
\end{itemize}

\blue{
Figure \ref{fig:pattrn} illustrates the tested MCM chiplet patterns across the different MCM systems. We test heterogeneous patterns including checkerboards (Het-CB), Sides (Het-Sides), Cross (Het-Cross). The 3$\times$3 MCM patterns are the default. }

\betterparagraph{Optimization Targets} We perform our search space exploration experiments to target optimizing a single metric at a time, coining the terms Latency Search, Energy Search, and EDP Search. EDP Search is our default experiment.
% The search experiments can be configured using $\gamma$ values in Equation \ref{eqn:scores}, setting it $\gamma$=1 for the target metric and zero for all others. EDP Search is our default experiment.

\betterparagraph{Search Criteria}
We adopt an exhaustive brute-force search for all experiments entailing the $3\times3$ MCM template. For the scaled $6\times6$ experiment, we implement a meta heuristic evolutionary algorithm for the SEG module to navigate the rising complexity. We set the population size and max number of generations to 10 and 4, respectively. 

% The evaluation criteria follows the scoring function based on hierarchical latency and energy models derived in Section \ref{sec:problem_formulation}.


% \betterparagraph{Search Space Parameters} At the \textit{MCM-Reconfig} level, we set the default $n_{splits}$ to 4 (i.e., 5 candidate reconfiguration windows), and $n_{cand}$ to 15 as the MCM-Reconfig search space characterization. We constrain the number of resources assigned to a model workload within a single time window to 6 (recall heuristic in Section \ref{subsec:segment}).

% \betterparagraph{LLMs Optimization Horizon} Given the repetitive, identical, and isomorphic (i.e., same input/output sizes) nature of LLM layers -- where an LLM layer constitutes a number of sub-layers (e.g., attention heads and linear layers) \cite{vaswani2017attention, devlin2018bert, brown2020language}, we limit the number of LLM layers within a single problem's optimization horizon to those that yield a comparable computational footprint to the remaining models in the multi-model inference scenario. This is driven by the sheer disparity in computational footprint between LLMs and other classes of models, and applying this approach enables us to explore finer-grained scheduling candidates across the multi-model suite without severely compounding the search space. In accordance, the remaining unconsidered LLM layers can be treated as separate sub-problems whose configurations can be combined to form their full computing schedules. Appendix?

% \textbf{Compute Cluster}

% l heterogeneous MCM architectures that have memory interfaces at the left and right sides, as illustrated in the ouptut of ~\autoref{fig:Overview}. Each chiplet on the left- and right-most columns possess a direct link to the offchip DRAM via double sided memory channels. We construct a cost model considering the NoP and offchip communication overheads utilizing the architectural parameters from \cite{shao2019simba, orenes2023massive} as shown in Table \ref{tab:params}. 

\begin{figure}[!tbp]
\begin{center}
{\includegraphics[,width = 0.48\textwidth]{Figures/pareto_5_3_5_sngl.pdf}}
\end{center}
\vspace{-2.6ex}
    \caption{Comparing brute force scheduling space exploration processes across various MCM configurations for various search targets for scenarios 4 and 5 from Table \ref{tab:scenarios}. 
    % The energy and latency evaluations for every explored point from the scheduling space are displayed for the variations of the 3$\times$3 MCM configurations in Figure \ref{fig:pattrn}. 
    \textit{standalone Shi-diannao} and \textit{standalone NVDLA} indicate cases where execution is performed on a single chiplet supporting said dataflow. }
\label{fig:pareto}
% \vspace{-3ex}
\end{figure}

\begin{figure}[!tbp]
\begin{center}
{\includegraphics[,width = 0.48\textwidth]{Figures/vr_pareto.pdf}}
\end{center}
\vspace{-2ex}
    \caption{Pareto optimal results on the EDP search experiments for the labeled XRBench usage scenarios. Results normalized by standalone NVDLA}
\label{fig:vr_pareto}
% \vspace{-3ex}
\end{figure}

\subsection{Search Space Exploration Analysis}

\input{Tables/results_breakdown}

\input{Tables/results_breakdown_vr}

We compare the $3\times3$ MCM brute-force search experiments for the heterogeneous and baseline configurations across the different optimization targets. Normalized performance estimates are evaluated relative to the standalone NVDLA baseline. Our experimental results for the MLPerf and AR/VR multi-model scenarios are provided in Tables \ref{tab:breakdown} and \ref{tab:breakdown_vr}, and we illustrate the Pareto plots across the different search experiments for Scenarios 3,4 and 4 and subset of the AR/VR experiments in the respective Figures \ref{fig:pareto} and \ref{fig:vr_pareto}, from which we discuss our findings as follows:

\betterparagraph{Pipelining Speedups} We observe that the combination of pipelining and chiplet heterogeneity lead to Pareto-optimal operating points that offer performance improvement opportunities. In Figure \ref{fig:pareto}, we see that pipelining individually can offer speedups over standalone baselines. \blue{For example, Scenario 3 (Latency Search) -- top-left most sub-Figure -- shows Simba (NVDLA) realizing configurations achieving up to 2.9$\times$ speedup over the standalone NVDLA as a result of multi-chiplet pipelining (The 1.37 compared to 4.06 ms in Table \ref{tab:breakdown}). The reason being that as our scheduler targets latency optimization, it attempts to consistently identify chiplet assignment strategies that equate pipelining latencies between model workloads assigned to the same window via inter-chiplet pipelining. For instance, in the time window at which the ResNet-50 concludes execution, the scheduler queued 18, 14, and 29 layers from the GPT-L, BERT-L, and ResNet-50 for processing, provisioned 3 chiplets for each model subset, and yielded accordingly 3 layer segments per model to be distributed across the 3 assigned chiplets, and achieve comparable latencies of 0.28 ms, 0.32, and 0.33 ms through applying inter-chiplet pipelining when applicable. The analysis is repeated across all time windows to realize the 1.37 ms.
Additionally, keeping quite a few, medium-sized data traffic from the (32-batch ResNet-50) on package via chiplet-to-chiplet data passing offers additional energy savings by avoiding a number of offchip memory R/W accesses at the start/finish of layer segments' execution. }

\betterparagraph{Heterogeneous Integration Synergy} As the density of multi-model workloads increase (Scenario 4 from Figure \ref{fig:pareto}), we observe the effectiveness of homogeneous pipelining drops due to the increased competition for chiplet resources from heavier workloads. Heterogeneous MCM solutions become viable in such cases as they add another dimension for boosting performance through heterogeneous pipelining schedules, which compensate for the rising complexity through considering the varying affinities of diverse model layers, improving both latency and energy efficiency as seen in their respective search experiments. This benefits of heterogeneous pipelining also hold for the AR/VR scenarios as seen by up to $1.25\times$ execution speedups in Figure \ref{fig:vr_pareto}. \\
\betterparagraph{Model Suite Diversity} The degree of diversity within the multi-model use-case also influences the overall performance improvement. In Scenario 3 (Figure \ref{fig:pareto} top), GPT-L and BERT-L were dominant transformer-based workloads with strong affinities towards the NVDLA dataflow style, contributing to the homogeneous Simba (NVDLA) solutions dominating the Pareto frontier. Scenario 4 (Figure \ref{fig:pareto} bot) and the AR/VR (Figure \ref{fig:vr_pareto}), more diversification of the layer workloads set lead more heterogeneous pipelining solutions to dominate the Pareto frontier. \\
\betterparagraph{Target Optimization} As illustrated in Figure \ref{fig:pareto}, the dominance of MCM configurations is also dependent on the target optimization metric. For instance in Figure \ref{fig:pareto} Scenario 4, the Standalone NVDLA baseline is the most energy-efficient solution as it does not incur NoP data movement costs from pipelining. However for Energy Search experiment, Het-Sides configuration identifies scheduling solutions that become the most energy efficient ones by leveraging heterogeneity to overcome extra NoP costs.

% NOTE: One explanation for pipelining being more energy efficient than standalone is due the residual connections of the resent enforce additional write back and fetch to the offchip memory, whereas pipelining options facilitate them being existant in other chiplets, which is less costly.

\begin{figure}[!tbp]
\begin{center}
{\includegraphics[,width = 0.48\textwidth]{Figures/barplots_5_3_5.pdf}}
\end{center}
\vspace{-3ex}
    \caption{Latency, energy, and EDP evaluations for the top-scoring candidates normalized by the standalone NVDLA for every datacenter scenario.
    }
\label{fig:barplots}
% \vspace{-3ex}
\end{figure}


\begin{figure}[!tbp]
\begin{center}
{\includegraphics[,width = 0.48\textwidth]{Figures/vr_barplot_2.pdf}}
\end{center}
\vspace{-2ex}
    \caption{Evaluations on the EDP search for the XRBench usage scenarios listed in Table \ref{def:workload_scenario} normalized by NVDLA standalone configuration.}
\label{fig:vr_barplot}
% \vspace{-3ex}
\end{figure}

\subsection{Top Performing Schedules Comparison}

We compare the top-performing scheduling configurations for each MCM configuration across the various scenarios.

\betterparagraph{NoP and Inter-chiplet Pipelining} We take barplot A1 in Figure \ref{fig:barplots} as an example and and zoom in on the Simba (NVDLA) configuration (2nd category) in each scenario. In Scenarios 1-3, the small number of models and limited diversity lead the benefits of inter-chiplet pipelining to outweigh the added NoP costs, enhancing throughput and achieving latency speedups over the standalone NVDLA baseline reaching $1.4\times$, $1.4\times$, $3.3\times$, respectively. Scenarios 4 and 5 sustain larger NoP overheads due to the increased traffic contention from more workloads, causing Simba (NVDLA) $1.05\times$ slowdown compared to the baseline in both scenarios.

% 5,3,5 configuration 
% Latency Search: 'hom_kcp': [0.702, 0.749, 0.337, 1.05, 1.051]
% [1.4, 1.4, 3.3, 0.95, .95]


% oled
% 1.4$\times$, 1.3$\times$, and 1.8$\times$ factors,


\betterparagraph{Heterogeneity Pattern Choices} 
Across the heterogeneous MCM scheduling options in Figure \ref{fig:barplots} (Het-CB and Het-Sides), we notice that in the majority of cases, Het-Sides outperforms Het-CB. The reason being is that Het-Sides presents workloads with inter-chiplet pipelining options that can either be homogeneous or heterogeneous based on the chiplets heterogeneous arrangement . This is especially beneficial in cases where are sequences of layers that can benefit from pipelining while sharing the same dataflow affinities, unlike Het-CB which can only offer the heterogeneous pipelining option. 
% \red{LC: is this primarily contributed by the better spatial locality of the Het-sides compared to Het-CB}.

\betterparagraph{Scenario and Optimization Target} In all matching criteria plots (A1, B2, and C3), Het-Sides configuration at the most compute-intensive and diverse scenarios 4 and 5 consistently outperforms all baselines. For example, Scenario 4 EDP in barplot C3 is reduced by factors of 2.3$\times$ and 2.6$\times$ compared to Simba (NVDLA) and Simba (Shi-diannao), respectively, while being 9.25$\times$ less than the standalone NVDLA.
We also show in Figure \ref{fig:vr_barplot} the matching EDP barplot for the AR/VR experiments. We observe that Het-Sides
option remains the most efficient option compared to the Simba baselines, achieving on average $5.2\%$ improvement over the standalone NVDLA. 

% 'edp': {'het_cb': [0.68, 0.785, 0.212, 0.151, 0.199], 'het_sides': [0.51, 0.649, 0.276, 0.108, 0.149], 'hom_kcp': [0.442, 0.509, 0.129, 0.253, 0.262], 'hom_ykp': [1.735, 1.883, 0.152, 0.278, 0.374]}}

% AR/VR
% het_sides_avg = 0.1918
% 'edp': {'het_cb': [0.294, 0.25, 0.18, 0.115, 0.169], 'het_sides': [0.267, 0.232, 0.179, 0.116, 0.165], 'hom_kcp': [0.283, 0.24, 0.222, 0.223, 0.209], 'hom_ykp': [0.51, 0.482, 0.262, 0.125, 0.371]}}
% [0.267, 0.232, 0.179, 0.116, 0.165]

% \begin{figure*}[!tbp]
% \begin{center}
% {\includegraphics[,width = 0.98\textwidth]{Figures/squeeze_sc_4_edp_top_cand.pdf}}
% \end{center}
% \vspace{-1ex}
%     \caption{Illustration of the top-scoring partitioning strategy for the scenario 4 experiments given the heterogeneous-sides configuration. Each window showcases the top-performing schedule within, and the mapping of models onto chiplets. Time boundaries between successive windows are computed over 500 MHz.}% times for MCM reconfiguration and new window initiation are computed over a 500 MHz operating frequency and displayed on top between each successive time windows.}
% \label{fig:top_cand}
% \vspace{-3ex}
% \end{figure*}

\begin{figure}[!tbp]
\begin{center}
{\includegraphics[,width = 0.49\textwidth]{Figures/sc_4_top.pdf}}
\end{center}
\vspace{-3ex}
    \caption{Illustration of the top-scoring scheduling strategy for Scenario 4 Het-Sides. Allocaiton of chiplets and and coarse-grained schedules are shown for each time window. Times computed over 500 MHz indicate the cumulative latency until the respective window concludes execution.}
\label{fig:top_cand}
\vspace{-3ex}
\end{figure}

\betterparagraph{Het-Sides Top Scheduling Strategy} In Figure \ref{fig:top_cand}, we illustrate the overall scheduling strategy for the top-scoring Het-Sides solution from the EDP search in Scenario 4. The Figure depicts the per-window inner schedules and the progression of accumulative latency for processing the workloads packed into each window. The distinguishing feat from this top scheduling strategy is the non-uniformity of time windows resulting from the greedy-packing heuristic, where smaller workloads (ResNet-50) are assigned to the earlier windows at the expense of larger workloads (e.g., from BERT-L) being delayed to subsequent windows. This facilitates (i) optimizing the schedules of smaller workloads at a finer level of granularity; (ii) avoiding starvation of smaller workloads. Starting from window 2, GPT-L and BERT workloads dominate the schedule, having their segmentation and mapping strategies optimized to minimize the experienced EDP in each window. In Table \ref{tab:top_lat}, we breakdown how the latency of each window is estimated alongside their assigned number of layers.


\input{Tables/top_lat}

\begin{figure}[!tbp]
\begin{center}
{\includegraphics[,width = 0.48\textwidth]{Figures/ablation_2x3.pdf}}
\end{center}
\vspace{-3ex}
    \caption{Results for the top performing schedule for the EDP Search for Scenarios 3 and 4 on the Triangular Patterns from Figure \ref{fig:pattrn}.}

\label{fig:ablation_2x3}
% \vspace{-3ex}
\end{figure}

\subsection{Ablation on Windowing and Chiplets Scaling}

\betterparagraph{Ablation Study on Time Partitioning}Using Scenario 4 and Het-Sides EDP Search experiments, we study how performance changes when varying $n_{splits}$ and repeating the experiment in Figure \ref{fig:split_sweep}. We observe the rate of EDP improvements starts to plateau after $n_{splits}$=4 similar to our analysis in Figure \ref{fig:mcm_config_opt}, where EDP of the top candidate is reduced from $n_{splits}$=4 to $n_{splits}$=5 by a factor of 1.04$\times$. %at the expense of 26.5$\times$ search time increase. 
% more reconfiguration provides finer specialization/adaptability of the MCM to the underlying workloads at the expense of reconfiguration overhead.

% Search Times
% 3286083 s for nsplits =5
% 123622 s for nsplits = 4

\blue{
\betterparagraph{{Ablation Study on other NoP Topology}}We study how SCAR generalizes to other topologies by performing the EDP search for Scenarios 3 and 4 using the the triangular NoP templates from Figure \ref{fig:pattrn}. As shown in Figure \ref{fig:ablation_2x3}, the top performing schedule from each scenario exhibits similar performance patterns compared to the original Scenario results on the 3$\times$3 Mesh, albeit with different relative evaluations. For instance, though our heterogeneous configuration outperforms both Simba-T strategies in Scenario 4 by 2.5$\%$ and 1.67$\%$ over Simba-T (Shi) and Simba-T (NVD), respectively, it is second best compared to Simba-T (NVD) in Scenario 3 by a 2.5$\%$ (\red{get corrected number})unlike in the $3\times3$ template in which it outperformed). This can be attributed to Scenario 3 being more affine towards NVD, and the tested Het-T template did not posses as many NVD chiplets as the $3\times3$ MCM). This further reinforces our insight that understanding the workload is instrumental in identifying the top-performing hardware parameter knobs.}

\blue{
\betterparagraph{{Ablation Study on PROV expected values}} We repeated the EDP search for Scenarios 3, 4, and, 5 on the $3\times3$ template using an exhaustive search over the $N_i$ Provisioner values as an ablation on the effectiveness of uniform resource distribution heuristic from Equation \ref{eqn:expectation}. In a similar following to the heuristic's results in Table \ref{tab:breakdown}, the Exhaustive search had Simba (NVD) as the top template for Scenario 3, while Het-Sides was superior at Scenarios 4 and 5, achieving \red{59.5\%, x} over Simba (Shi), \red{33.0\%, x} EDP reduction in EDP over Simba (NVD). 
}


We studied how the uniform resource distribution by the Provisioner in Equation \ref{eqn:expectation} follows an exhaustive over all possible values of $N_i$. We performed an exhaustive EDP search for Scenarios 3, 4, and, 5 on the $3\times3$ template. 

\betterparagraph{Ablation on Greedy Packing Algorithm} Using Scenario 4 and Het-Sides configuration, We tested the efficacy of our first-fit greedy layer packing algorithm against a uniform packing baseline, which uniformly distributes layers from each model across time windows in a uniform fashion. The Greedy layer packing algorithm was superior, improving execution speedups and energy efficiency by 21.8\% and 8.6\%, respectively.

\betterparagraph{Scalability}
\blue{We assess how SCAR scales with the hardware using the 6$\times$6 full Simba MCM system with its templates from Figure \ref{fig:pattrn}.} We implement an evolutionary algorithm for the \textit{SEG} engine to scale with the problem size, and show the results for the EDP search on Scenario 4 at $n_{splits}$=$2$ and $n_{splits}$=$3$. \blue{We choose the heterogeneous cross (Het-Cross) as our heterogeneous template following the insights from the 3$\times$3 experiment regarding choosing heterogeneity patterns that enable both homogeneous and heterogeneous pipelining capabilities.} As shown in Figure \ref{fig:ea_barplot}, the evolutionary search has led to identifying configurations for Het-Cross that achieve 2.3$\times$ and 1.9$\times$ reduction in EDP; 2.1$\times$ and 1.8$\times$ reduction in latency over Simba (Shi) and Simba (NVD), respectively.


% We assess the scalability of our search framework using the full 6$\times$6 Simba MCM system, where we implement an evolutionary algorithm for the \textit{SEG} considering the rising problem complexity from the inclusion of more chiplets. We perform the search for our default experimental settings and Scenario 4 given $n_{splits}\in\{2,3\}$. We employ a Heterog-Cross pattern and compare it against the Simba baselines in Figure \ref{fig:ea_barplot}. We find that the Heterog-Cross top-scoring schedule outperforms those from the Simba baselines in all cases across all metrics. At $n_{splits}$=3, Heterog-Cross leads to 2.3$\times$ and 1.9 $\times$ reduction in EDP; 2.1$\times$ and 1.8$\times$ reduction in latency; over Simba (Shi-diannao) and Simba (NVDLA) and, respectively.


\begin{figure}[!tbp]
\begin{center}
\centering
{\includegraphics[width = .35\textwidth]{Figures/split_sweep.pdf}}
\end{center}
\vspace{-1.5ex}
    \caption{Sweep of $n_{splits}$ for the $3\times3$ Heterog-Sides MCM configuration under EDP search showing EDP and latency results for each case's top choice.}
\label{fig:split_sweep}
% \vspace{-3ex}
\end{figure}


% \begin{figure}[!tbp]
% \begin{center}
% {\includegraphics[,width = 0.45\textwidth]{Figures/ea_barplot.pdf}}
% \end{center}
% % \vspace{-1ex}
%     \caption{Comparing EDP and Latency at $n_{splits} \in \{2, 3\}
%     $ for the $6\times6$ MCM for target EDP optimizaiton and an evolutionary search algorithm.}
% \label{fig:ea_barplot}
% % \vspace{-3ex}
% \end{figure}

\begin{figure}[!tbp]
\begin{center}
{\includegraphics[,width = 0.48\textwidth]{Figures/ea_plots.pdf}}
\end{center}
\vspace{-3ex}
    \caption{Pareto Plot and comparison of top performing models for the EDP search on the $6\times6$ MCM at $n_{splits}$=2 (\textit{top}) and $n_{splits}$=3 (\textit{bot}). }

\label{fig:ea_barplot}
% \vspace{-3ex}
\end{figure}




==> Tables/top_edp.tex <==
\begin{table}[t]
    \centering
    \caption{EDP Evaluations breakdown in \textbf{J.seconds} for the top partitioning candidate from Scenario 4 EDP Search across all its time windows.}
    \vspace{-2ex}
    \begin{tabular}{ l | c  c  c  c  c |c | }
    \hline
     & \textbf{W0} & \textbf{W1} & \textbf{W2} & \textbf{W3} & \textbf{W4} & \textbf{tot} \\
    \hline
    \textbf{GPT-L} & 0.23 & 0.21 & 1.02 & 0.28 & 0.23 & 1.97 & 4.2 \\ 
    \textbf{BERT-L} & 0 & 0 & 1.47 & 0.4 & 0.90 & 2.77 & 4.95 \\
    \textbf{U-Net} & 0.21 & 0.13 & 0.46 & 0 & 0 & 0.8 & 2.71 \\
    \textbf{ResNet} & 0.78 & 0.17 & 0.11 & 0 & 0 & 1.1 & 2.36 \\
    \hline
    \textbf{accum.} & 0.78 & 1.47 & 1.4 & 0.4 & 0.9 & - &  4.95\\ 
    \hline
    \end{tabular}
    \label{tab:top_lat}
    \vspace{-3ex}
\end{table}
